On the Application of ISO 26262 in Control Design for Automated Vehicles

Research on automated vehicles has experienced an explosive growth over the past decade. A main obstacle to their practical realization, however, is a convincing safety concept. This question becomes ever more important as more sophisticated algorithms are used and the vehicle automation level increases. The field of functional safety offers a systematic approach to identify possible sources of risk and to improve the safety of a vehicle. It is based on practical experience across the aerospace, process and other industries over multiple decades. This experience is compiled in the functional safety standard for the automotive domain, ISO 26262, which is widely adopted throughout the automotive industry. However, its applicability and relevance for highly automated vehicles is subject to a controversial debate. This paper takes a critical look at the discussion and summarizes the main steps of ISO 26262 for a safe control design for automated vehicles.

==> eptcsdata.tex <==
\providecommand{\firstpage}{74}
\providecommand{\publicationstatus}{M. Gleirscher, S. Kugele, S. Linker (Eds.): 2nd International\\ Workshop on Safe Control of Autonomous Vehicles (SCAV 2018)\\
EPTCS 269, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.269.7}{10.4204/EPTCS.269.7}}

